Predictive Chemistry Augmented with Text Retrieval

This paper focuses on using natural language descriptions to enhance predictive models in the chemistry field. Conventionally, chemoinformatics models are trained with extensive structured data manually extracted from the literature. In this paper, we introduce TextReact, a novel method that directly augments predictive chemistry with texts retrieved from the literature. TextReact retrieves text descriptions relevant for a given chemical reaction, and then aligns them with the molecular representation of the reaction. This alignment is enhanced via an auxiliary masked LM objective incorporated in the predictor training. We empirically validate the framework on two chemistry tasks: reaction condition recommendation and one-step retrosynthesis. By leveraging text retrieval, TextReact significantly outperforms state-of-the-art chemoinformatics models trained solely on molecular data.

==> bak/background.tex <==
\section{Related Work}

\paragraph{Document Retrieval} 
This field studies algorithms for retrieving relevant documents from a large corpus in response to an information need (i.e., a query). In the context of natural language processing, both the query and document are natural language text. Traditional methods represent them as bag-of-words vectors, such as TF-IDF \cite{Jones04} and  BM25 \cite{BM25}. More recently, researchers proposed neural networks to learn latent vector representations for retrieval tasks \cite{LeeCT19,KarpukhinOMLWEC20}. The query and document are independently encoded with separate encoders, which are trained by contrastive learning on labeled (query, document) pairs. Afterward, the encodings of all the documents in the corpus are pre-computed and indexed, allowing for efficient retrieval using maximum inner product search \cite{MussmannE16}. 

Our work also focuses on retrieving relevant documents in response to a query, but the query is a chemistry input (e.g., a molecule or reaction) rather than natural language text. 

\paragraph{Retrieval-Augmented Language Models}
There have been several studies on augmenting language models with retrieval techniques. The idea is to retrieve relevant documents from a corpus and use them as additional context to the model. Earlier works on open-domain question answering adopted standalone retrievers to identify supporting paragraphs for the given questions \cite{ChenFWB17,KarpukhinOMLWEC20}. \citet{REALM} proposed REALM, which jointly trains an end-to-end retriever with a language model.  \citet{RAG} extended this idea to more general sequence-to-sequence generation tasks.

Our work shares a similar idea of retrieval augmentation. However, we focus on tasks in the predictive chemistry domain (see \Cref{fig:chemie,fig:chemtask}), where the goal is to develop machine learning models to help design new drugs or materials \cite{segler2018planning,doi:10.1126/science.aax1566,D0SC04184J}.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/tasks.pdf}
    \caption{Predictive chemistry tasks studied in this work. (a) Reaction condition recommendation. (b) One-step retrosynthesis.}
    \label{fig:chemtask}
\end{figure}


% \paragraph{Retrosynthesis}
% Retrosynthesis planning, a crucial task in the chemical and pharmaceutical industry, involves designing pathways for synthesizing target molecules from available starting chemicals. In recent years, machine learning methods have been applied in computer-aided synthesis planning (CASP) \cite{segler2018planning,doi:10.1126/science.aax1566,D0SC04184J}. These methods leverage neural networks to make predictions about chemical reactions, and use Monte Carlo tree search to explore and discover the retrosynthetic routes. In this work, we study two predictive chemistry tasks related to retrosynthesis, which are shown in \Cref{fig:chemtask}.


\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/textreact.pdf}
    % \vspace{-0.1in}
    \caption{Overview of \textreact. The retriever searches for relevant texts to the chemistry input, which are then used to augment the input of the predictor. This figure illustrates reaction condition recommendation as an example chemistry task. }
    \label{fig:textreact}
\end{figure*}


\paragraph{Reaction Condition Recommendation}
Reaction condition recommendation is the task of suggesting reaction conditions, such as catalysts, solvents, and reagents, for a chemical reaction. \citet{acscentsci.8b00357} proposed a machine learning model for this task, where the reaction is represented as the difference between the product and the reactant fingerprint vectors, indicating the change of substructures during the reaction, and the reaction conditions are sequentially predicted by the model. Later research studied different methods to represent the reaction, such as MACCS key fingerprints \cite{acs.jcim.9b00313} and graph neural networks \cite{ryou2020graph}, and alternative machine learning formulations, such as multilabel classification \cite{acs.jcim.0c01234} and variational inference \cite{acs.jcim.2c01085}. In this work, we follow \citeauthor{acscentsci.8b00357}'s formulation but use the more advanced Transformer architecture.



\paragraph{One-Step Retrosynthesis}
Another important task in predictive chemistry is one-step retrosynthesis, which aims to propose reaction precursors (reactants) for target molecules (products). Prior methods can be broadly classified into two categories: \textit{template-based} and \textit{template-free}. Template-based approaches use classification models to predict the reaction template that can be applied to the target \cite{chem.201605499,jacsau.1c00246}, and subsequently employ cheminformatics software to derive the precursors based on the template. Template-free approaches have a more ambitious goal: predicting the precursors directly without relying on a fixed set of reaction templates. Such approaches are usually implemented as graph-to-graph or sequence-to-sequence generation models \cite{acscentsci.7b00303,DaiLCDS19,ShiXG0T20,C9SC03666K,SomnathBCKB21}, and achieve comparable performance to template-based approaches on common benchmarks.
We adopt a template-free approach in this work, but our method also applies to template-based approaches.




==> bak/intro.tex <==
\section{Introduction}

In recent years, machine learning techniques have been widely used in predictive chemistry \cite{segler2018planning,chemprop,predictive_chemistry,wcms.1604}. Leveraging reaction data from the chemistry database, researchers train neural network models to predict molecular properties and reaction outcomes, and plan synthesis pathways. The scientific information extraction community has devoted decades of effort to the automation of constructing structured databases from the literature \cite{LiuHTWF06,chemicaltagger,lowe2012extraction,cde}.  However, this information extraction task presents significant challenges and complexities.  It necessitates specialized model architectures and substantial training data, and may not always generalize effectively to new extraction tasks or domains \cite{LuanHOH18,guo2021automated,RxnScribe}. These challenges make it difficult for the model to leverage the latest findings in the literature, thus impeding advancements in predictive chemistry. 

In this paper, we propose a novel framework, \textreact, which augments predictive chemistry tasks with text retrieval. As illustrated in \Cref{fig:chemie}, our approach directly retrieves relevant information for a chemistry task from a natural language corpus of chemical reactions, circumventing the intermediate information extraction step. The retrieved texts are utilized as supplementary input to augment the model's predictive capabilities. 

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/chemie2.pdf}
    % \vspace{-0.1in}
    \caption{Predictive chemistry augmented with text retrieval. Unlike conventional approach that extracts structured data first,  TextReact augments chemistry prediction by directly retrieving relevant text from the literature. }
    \label{fig:chemie}
\end{figure*}

\textreact addresses three computational challenges in leveraging natural language for chemistry prediction. First, to match a chemistry input with its corresponding text description, we train a dual-encoder retriever through contrastive learning. Second, we design a text-augmented predictor to integrate both the chemistry input and retrieved text, and incorporate an auxiliary masked language modeling objective to foster the model's understanding of the correlation between chemistry and text inputs. Third, we adopt a random sampling policy during training to simulate examples that can be found in the corpus as well as those that are not present within the corpus, such that the model generalizes to novel chemistry inputs.  While \textreact requires the same volume of training data as conventional chemistry-only models, it is enhanced with the ability to retrieve and utilize information from unlabeled text corpora. 

We experiment with two predictive chemistry tasks: (1) reaction condition recommendation, which involves recommending suitable conditions for a chemical reaction, and (2) one-step retrosynthesis, which involves predicting the reactants given a product molecule. In both tasks, our retriever shows strong performance in retrieving text relevant to the chemistry input. By leveraging text retrieval, \textreact achieves substantial performance improvements, increasing the top-1 prediction accuracy by 58.4\% for reaction conditions and 12.7\% for one-step retrosynthesis. The improvement is consistent under both random and time-based splits of the datasets, validating the efficacy of our retrieval augmentation approach in generalizing to different scenarios. The results demonstrate that for novel chemistry input lacking direct description in the corpus, retrieving information on similar reactions is also beneficial to the model. 
Our code and data will be publicly available upon publication.
% at \url{https://github.com/thomas0809/textreact}.

